Parasitic Circus:On the Feasibility of Golden Free PCB Verification

Printed circuit boards (PCBs) are an integral part of electronic systems. Hence, verifying their physical integrity in the presence of supply chain attacks (e.g., tampering and counterfeiting) is of utmost importance. Recently, tamper detection techniques grounded in impedance characterization of PCB's Power Delivery Network (PDN) have gained prominence due to their global detection coverage, non-invasive, and low-cost nature. Similar to other physical verification methods, these techniques rely on the existence of a physical golden sample for signature comparisons. However, having access to a physical golden sample for golden signature extraction is not feasible in many real-world scenarios. In this work, we assess the feasibility of eliminating a physical golden sample and replacing it with a simulated golden signature obtained by the PCB design files. By performing extensive simulation and measurements on an in-house designed PCB, we demonstrate how the parasitic impedance of the PCB components plays a major role in reaching a successful verification. Based on the obtained results and using statistical metrics, we show that we can mitigate the discrepancy between collected signatures from simulation and measurements.

==> Figures/references.tex <==
@article{luo2014method,
  title={Method for reliability parameter calculation of electronic products based on physics of failure models},
  author={Luo, MZ and Chen, Y and Kang, R},
  journal={Systems Engineering and Electronics},
  volume={36},
  number={4},
  pages={795--801},
  year={2014}
}
@article{mehta2020big,
  title={The big hack explained: Detection and prevention of PCB supply chain implants},
  author={Mehta, Dhwani and Lu, Hangwei and Paradis, Olivia P and MS, Mukhil Azhagan and Rahman, M Tanjidur and Iskander, Yousef and Chawla, Praveen and Woodard, Damon L and Tehranipoor, Mark and Asadizanjani, Navid},
  journal={ACM Journal on Emerging Technologies in Computing Systems (JETC)},
  volume={16},
  number={4},
  pages={1--25},
  year={2020},
  publisher={ACM New York, NY, USA}
}
@inproceedings{bhattacharyay2022vipr,
  title={{VIPR-PCB}: a machine learning based golden-free {PCB} assurance framework},
  author={Bhattacharyay, Aritra and Chakraborty, Prabuddha and Cruz, Jonathan and Bhunia, Swarup},
  booktitle={Proceedings of the 59th ACM/IEEE Design Automation Conference},
  pages={793--798},
  year={2022}
}
@article{candido2023image,
  title={Image-Based Detection of Modifications in Assembled PCBs with Deep Convolutional Autoencoders},
  author={Candido de Oliveira, Diulhio and Nassu, Bogdan Tomoyuki and Wehrmeister, Marco Aurelio},
  journal={Sensors},
  volume={23},
  number={3},
  pages={1353},
  year={2023},
  publisher={MDPI}
}
@inproceedings{andrade2021survey,
  title={A Survey on Automatic Inspection for Printed Circuit Board Analysis},
  author={Andrade, Marcos Ant{\^o}nio and Pepe, Pedro Carlos Fazolino and Ximenes, Leandro Ronchini and Arthur, Rangel},
  booktitle={Brazilian Technology Symposium},
  pages={423--431},
  year={2021},
  organization={Springer}
}
@article{abd2020review,
  title={A review and analysis of automatic optical inspection and quality monitoring methods in electronics industry},
  author={Abd Al Rahman, M and Mousavi, Alireza},
  journal={Ieee Access},
  volume={8},
  pages={183192--183271},
  year={2020},
  publisher={IEEE}
}
@article{zhang2022deep,
  title={Deep learning based solder joint defect detection on industrial printed circuit board X-ray images},
  author={Zhang, Qianru and Zhang, Meng and Gamanayake, Chinthaka and Yuen, Chau and Geng, Zehao and Jayasekara, Hirunima and Woo, Chia-wei and Low, Jenny and Liu, Xiang and Guan, Yong Liang},
  journal={Complex \& Intelligent Systems},
  volume={8},
  number={2},
  pages={1525--1537},
  year={2022},
  publisher={Springer}
}
@inproceedings{ivanova2021machine,
  title={Machine learning for in-circuit testing of printed circuit board assembly},
  author={Ivanova, Malinka and Petkov, Nikolay},
  booktitle={Proceedings of the 2021 4th Artificial Intelligence and Cloud Computing Conference},
  pages={221--228},
  year={2021}
}
@article{alaoui2019using,
  title={Using infrared thermal responses for PCBA production tests: Feasibility study},
  author={Alaoui, Nabil El Belghiti and Cassou, Anais and Tounsi, Patrick and Boyer, Alexandre and Viard, Arnaud},
  journal={Microelectronics Reliability},
  volume={100},
  pages={113354},
  year={2019},
  publisher={Elsevier}
}
@article{denon,
  title={Non-intrusive Embedded Systems Anomaly Detection using Thermography and Machine Learning},
  author={de Oliveira, Jos{\'e} Paulo G and Bastos Filho, Carmelo JA and Oliveira, S{\'e}rgio Campello}
}
@article{adibhatla2020defect,
  title={Defect detection in printed circuit boards using you-only-look-once convolutional neural networks},
  author={Adibhatla, Venkat Anil and Chih, Huan-Chuang and Hsu, Chi-Chang and Cheng, Joseph and Abbod, Maysam F and Shieh, Jiann-Shing},
  journal={Electronics},
  volume={9},
  number={9},
  pages={1547},
  year={2020},
  publisher={MDPI}
}
@article{farahmandi2020hardware,
  title={Hardware {T}rojan detection schemes using path delay and side-channel analysis},
  author={Farahmandi, Farimah and Huang, Yuanwen and Mishra, Prabhat and Farahmandi, Farimah and Huang, Yuanwen and Mishra, Prabhat},
  journal={System-on-Chip Security: Validation and Verification},
  pages={221--271},
  year={2020},
  publisher={Springer}
}
@inproceedings{rad2008sensitivity,
  title={Sensitivity analysis to hardware {T}rojans using power supply transient signals},
  author={Rad, Reza and Plusquellic, Jim and Tehranipoor, Mohammad},
  booktitle={2008 IEEE International Workshop on Hardware-Oriented Security and Trust},
  pages={3--7},
  year={2008},
  organization={IEEE}
}
@inproceedings{narasimhan2011tesr,
  title={TeSR: A robust temporal self-referencing approach for hardware {T}rojan detection},
  author={Narasimhan, Seetharam and Wang, Xinmu and Du, Dongdong and Chakraborty, Rajat Subhra and Bhunia, Swarup},
  booktitle={2011 IEEE International Symposium on Hardware-Oriented Security and Trust},
  pages={71--74},
  year={2011},
  organization={IEEE}
}
@inproceedings{liu2014hardware,
  title={Hardware {T}rojan detection through golden chip-free statistical side-channel fingerprinting},
  author={Liu, Yu and Huang, Ke and Makris, Yiorgos},
  booktitle={Proceedings of the 51st Annual Design Automation Conference},
  pages={1--6},
  year={2014}
}

@inproceedings{xue2016enhanced,
  title={An enhanced classification-based golden chips-free hardware {T}rojan detection technique},
  author={Xue, Mingfu and Wang, Jian and Hu, Aiqun},
  booktitle={2016 IEEE Asian Hardware-Oriented Security and Trust (AsianHOST)},
  pages={1--6},
  year={2016},
  organization={IEEE}
}

@article{siwave,
    title = {New Integrated Workflow for {EMI} Simulation},
    author={Benson Wei and Steven G. Pytel Jr},
    journal={APEMC 2015}
   
}
@misc{ansys_siwave_2023,
  title = {{ANSYS SIwave 2023 R2}},
  author = {{ANSYS, Inc.}},
  year = {2023},
  howpublished = {\url{http://www.ansys.com}}
}

@inproceedings{yang2021research,
  title={Research on Signal Integrity in High-Speed Interconnection Channel Based on SIwave},
  author={Yang, Zheng and Gao, Yingke and Li, Shenglong and Sun, Chuanchuan and Zhao, Yunfu},
  booktitle={2021 IEEE 3rd International Conference on Circuits and Systems (ICCS)},
  pages={78--82},
  year={2021},
  organization={IEEE}
}

@article{zhu2023pdnpulse,
  title={{PDNP}ulse: sensing {PCB} anomaly with the intrinsic power delivery network},
  author={Zhu, Huifeng and Shan, Haoqi and Sullivan, Dean and Guo, Xiaolong and Jin, Yier and Zhang, Xuan},
  journal={IEEE Transactions on Information Forensics and Security},
  year={2023},
  publisher={IEEE}
}
@inproceedings{hashino2010characterization,
  title={Characterization of parasitic impedance in a power electronics circuit board using TDR},
  author={Hashino, Satoshi and Shimizu, Toshihisa},
  booktitle={The 2010 International Power Electronics Conference-ECCE ASIA-},
  pages={900--905},
  year={2010},
  organization={IEEE}
}


@article{mosavirik2023silicon,
  title={Silicon Echoes: Non-Invasive {T}rojan and Tamper Detection using Frequency-Selective Impedance Analysis},
  author={Mosavirik, Tahoura and Monfared, Saleh Khalaj and Safa, Maryam Saadat and Tajik, Shahin},
 journal={IACR Transactions on Cryptographic Hardware and Embedded Systems},
pages={238-261},
year={2023}
}


@inproceedings{amin2008speech,
  title={Speech recognition using dynamic time warping},
  author={Amin, Talal Bin and Mahmood, Iftekhar},
  booktitle={2008 2nd international conference on advances in space technologies},
  pages={74--79},
  year={2008},
  organization={IEEE}
}

@article{vintsyuk1968speech,
  title={Speech discrimination by dynamic programming},
  author={Vintsyuk, Taras K},
  journal={Cybernetics},
  volume={4},
  number={1},
  pages={52--57},
  year={1968},
  publisher={Springer}
}

@article{sakoe1978dynamic,
  title={Dynamic programming algorithm optimization for spoken word recognition},
  author={Sakoe, Hiroaki and Chiba, Seibi},
  journal={IEEE transactions on acoustics, speech, and signal processing},
  volume={26},
  number={1},
  pages={43--49},
  year={1978},
  publisher={IEEE}
}

@article{mosavirik2023impedanceverif,
  title={Impedanceverif: On-chip impedance sensing for system-level tampering detection},
  author={Mosavirik, Tahoura and Schaumont, Patrick and Tajik, Shahin},
  journal={IACR Transactions on Cryptographic Hardware and Embedded Systems},
  pages={301--325},
  year={2023}
}
@inproceedings{wang2009response,
  title={Response prediction and verification for PCB with package due to thermal and random vibration coupling effects},
  author={Wang, Bor-Tsuen and Hsu, Fu-Xiang and Liang, Xiu-Wei and Hung, Chen-Hsiung and Lai, Yi-Shao and Yeh, Chang-Lin and Lee, Ying-Chih},
  booktitle={2009 4th International Microsystems, Packaging, Assembly and Circuits Technology Conference},
  pages={401--404},
  year={2009},
  organization={IEEE}
}
@article{fujimoto2018demonstration,
  title={A demonstration of a HT-detection method based on impedance measurements of the wiring around ICs},
  author={Fujimoto, Daisuke and Nin, Shota and Hayashi, Yu-Ichi and Miura, Noriyuki and Nagata, Makoto and Matsumoto, Tsutomu},
  journal={IEEE Transactions on Circuits and Systems II: Express Briefs},
  volume={65},
  number={10},
  pages={1320--1324},
  year={2018},
  publisher={IEEE}
}
@inproceedings{safa2023counterfeit,
  title={Counterfeit Chip Detection using Scattering Parameter Analysis},
  author={Safa, Maryam Saadat and Mosavirik, Tahoura and Tajik, Shahin},
  booktitle={2023 26th International Symposium on Design and Diagnostics of Electronic Circuits and Systems (DDECS)},
  year={2023},
  organization={IEEE}
}
@article{mosavirik2022scatterverif,
  title={Scatterverif: Verification of electronic boards using reflection response of power distribution network},
  author={Mosavirik, Tahoura and Ganji, Fatemeh and Schaumont, Patrick and Tajik, Shahin},
  journal={ACM Journal on Emerging Technologies in Computing Systems (JETC)},
  volume={18},
  number={4},
  pages={1--24},
  year={2022},
  publisher={ACM New York, NY}
}

@article{big_hack,
  title={{The Big Hack: How China used a Tiny Chip to Infiltrate US Companies}},
  author={Robertson, Jordan and Riley, Michael},
  journal={Bloomberg Businessweek},
  volume={4},
  year={2018}
}

@article{fake_cisco,
  title={{The Fake Cisco: Hunting for Backdoors in Counterfeit Cisco Devices}},
  author={Janushkevich, Dmitry},
  journal={F-Secure Consulting, Hardware Security Team},
  year={2020}
}

@article{krishnamurthy2022multi,
  title={Multi-Modal Side Channel Data Driven Golden-Free Detection of Software and Firmware {T}rojans},
  author={Krishnamurthy, Prashanth and Surabhi, Virinchi Roy and Pearce, Hammond and Karri, Ramesh and Khorrami, Farshad},
  journal={IEEE Transactions on Dependable and Secure Computing},
  year={2022},
  publisher={IEEE}
}

@article{chowdhury2023golden,
  title={A Golden-Free Approach to Detect {T}rojans in {COTS} Multi-{PCB} Systems},
  author={Chowdhury, Animesh Basak and Mahapatra, Anushree and Liu, Yang and Krishnamurthy, Prashanth and Khorrami, Farshad and Karri, Ramesh},
  journal={IEEE Micro},
  year={2023},
  publisher={IEEE}
}
@article{asadizanjani2017pcb,
  title={PCB reverse engineering using nondestructive X-ray tomography and advanced image processing},
  author={Asadizanjani, Navid and Tehranipoor, Mark and Forte, Domenic},
  journal={IEEE Transactions on Components, Packaging and Manufacturing Technology},
  volume={7},
  number={2},
  pages={292--299},
  year={2017},
  publisher={IEEE}
}
@article{lu2020fics,
  title={Fics-pcb: A multi-modal image dataset for automated printed circuit board visual inspection},
  author={Lu, Hangwei and Mehta, Dhwani and Paradis, Olivia and Asadizanjani, Navid and Tehranipoor, Mark and Woodard, Damon L},
  journal={Cryptology ePrint Archive},
  year={2020}
}
@article{nguyen2019creating,
  title={Creating a backscattering side-channel to enable detection of dormant hardware Trojans},
  author={Nguyen, Luong N and Cheng, Chia-Lin and Prvulovic, Milos and Zaji{\'c}, Alenka},
  journal={IEEE transactions on very large scale integration (VLSI) systems},
  volume={27},
  number={7},
  pages={1561--1574},
  year={2019},
  publisher={IEEE}
}

@article{werner2022detection,
  title={Detection of recycled {ICs} using backscattering side-channel analysis},
  author={Werner, Frank T and Prvulovic, Milos and Zaji{\'c}, Alenka},
  journal={IEEE Transactions on Very Large Scale Integration (VLSI) Systems},
  volume={30},
  number={9},
  pages={1244--1255},
  year={2022},
  publisher={IEEE}
}


@article{awal2022nearfield,
  title={Nearfield RF sensing for feature-detection and algorithmic classification of tamper attacks},
  author={Awal, Md Sadik and Madanayake, Arjuna and Rahman, Md Tauhidur},
  journal={IEEE Journal of Radio Frequency Identification},
  volume={6},
  pages={490--499},
  year={2022},
  publisher={IEEE}
}

@article{piliposyan2022pcb,
  title={{PCB} Hardware {T}rojan Run-Time Detection Through Machine Learning},
  author={Piliposyan, Gor and Khursheed, Saqib},
  journal={IEEE Transactions on Computers},
  year={2022},
  publisher={IEEE}
}

@article{erai,
  title={{2019 ERAI Reported Parts Statistics}},
  author={{Akhoundov, Damir}},
  journal = {ERAI Blog},
  howpublished = "\url{https://www.erai.com/erai_blog/3167/2019_erai_reported_parts_statistics}",
  year={2020} 
}

@inproceedings{chaudhary2017automatic,
  title={Automatic visual inspection of printed circuit board for defect detection and classification},
  author={Chaudhary, Vikas and Dave, Ishan R and Upla, Kishor P},
  booktitle={2017 International Conference on Wireless Communications, Signal Processing and Networking (WiSPNET)},
  pages={732--737},
  year={2017},
  organization={IEEE}
}

@article{botero2021hardware,
  title={Hardware trust and assurance through reverse engineering: A tutorial and outlook from image analysis and machine learning perspectives},
  author={Botero, Ulbert J and Wilson, Ronald and Lu, Hangwei and Rahman, Mir Tanjidur and Mallaiyan, Mukhil A and Ganji, Fatemeh and Asadizanjani, Navid and Tehranipoor, Mark M and Woodard, Damon L and Forte, Domenic},
  journal={ACM Journal on Emerging Technologies in Computing Systems (JETC)},
  volume={17},
  number={4},
  pages={1--53},
  year={2021},
  publisher={ACM New York, NY}
}

